AttentionStitch: How Attention Solves the Speech Editing Problem

The generation of natural and high-quality speech from text is a challenging problem in the field of natural language processing. In addition to speech generation, speech editing is also a crucial task, which requires the seamless and unnoticeable integration of edited speech into synthesized speech. We propose a novel approach to speech editing by leveraging a pre-trained text-to-speech (TTS) model, such as FastSpeech 2, and incorporating a double attention block network on top of it to automatically merge the synthesized mel-spectrogram with the mel-spectrogram of the edited text. We refer to this model as AttentionStitch, as it harnesses attention to stitch audio samples together. We evaluate the proposed AttentionStitch model against state-of-the-art baselines on both single and multi-speaker datasets, namely LJSpeech and VCTK. We demonstrate its superior performance through an objective and a subjective evaluation test involving 15 human participants. AttentionStitch is capable of producing high-quality speech, even for words not seen during training, while operating automatically without the need for human intervention. Moreover, AttentionStitch is fast during both training and inference and is able to generate human-sounding edited speech.

==> neurips2023_workshop_sections/related_work.tex <==
% One approach is to generate prosody features around the edited speech area to control standard pitch-shift and time-stretch methods, while removing any artifacts caused by signal processing \cite{morrison2021context}. Another method, uses a generic voice to generate audio from the given text, which is then converted to a specific voice, inducing roughness at the boundaries of the edited audio \cite{jin2017voco}. EditSpeech \cite{tan2021editspeech} employs a partial inference process for the edited speech part using a bidirectional fusion process to make the boundaries smoother. A$^3$T \cite{bai20223}, learns to reconstruct masked areas in audio samples using text input and acoustic-text alignments. EdiTTS \cite{tae2021editts}, utilizes a diffusion model to apply edits only to targeted regions based on continuous perturbations in its Gaussian prior, but it is only evaluated in single speaker LJSpeech data. SpeechPainter \cite{borsos2022speechpainter}, synthesizes audio samples based on an unaligned text transcript, splitting the mel-spectrogram into patches. However, it is limited since it does not edit speech but fills up to 1 second gaps of speech with the missing reference text. MaskedSpeech \cite{zhang2022maskedspeech}, which is the closest approach to our method, is only applicable for speech editing on a sentence level and only for Mandarin speech data. Our proposed approach uses a pretrained model to reduce the need for additional training and employs an attention mechanism to edit speech automatically and smoothly.



